Towards Credential-based Device Registration in DApps for DePINs with ZKPs

Decentralized Physical Infrastructure Networks (DePINS) are secured and governed by blockchains but beyond crypto-economic incentives, they lack measures to establish trust in participating devices and their services. The verification of relevant device credentials during device registration helps to overcome this problem. However, on-chain verification in decentralized applications (dApp) discloses potentially confidential device attributes whereas off-chain verification introduces undesirable trust assumptions. In this paper, we propose a credential-based device registration (CDR) mechanism that verifies device credentials on the blockchain and leverages zero-knowledge proofs (ZKP) to protect confidential device attributes from being disclosed. We characterize CDR for DePINs, present a general system model, and technically evaluate CDR using zkSNARKs with Groth16 and Marlin. Our experiments give first insights into performance impacts and reveal a tradeoff between the applied proof systems.

==> __latexindent_temp.tex <==
@inproceedings{demystifyingOauth,
  title={OAuth Demystified for Mobile Application Developers},
  author={Eric Y. Chen and Yutong Pei and Shuo Chen and Yuan Tian and Robert Kotcher and Patrick Tague},
  booktitle={ACM Conference on Computer and Communications Security},
  year={2014}
}

@article{selfishMining_1,
author = {Eyal, Ittay and Sirer, Emin},
year = {2018},
month = {06},
pages = {95-102},
title = {Majority Is Not Enough: Bitcoin mining is vulnerable},
volume = {61},
journal = {Communications of the ACM},
doi = {10.1145/3212998}
}

@unknown{truebit,
author = {Teutsch, Jason and Reitwießner, Christian},
year = {2019},
month = {08},
title = {A scalable verification solution for blockchains}
}

@article{incentCorrectComp,
author = {Kumaresan, Ranjit and Bentov, Iddo},
year = {2014},
month = {11},
pages = {30-41},
title = {How to Use Bitcoin to Incentivize Correct Computations},
journal = {Proceedings of the ACM Conference on Computer and Communications Security},
doi = {10.1145/2660267.2660380}
}

@article{fairAccess_iot,
author = {Ouaddah, Aafaf and Elkalam, Anas and Ouahman, Abdellah},
year = {2017},
month = {02},
pages = {},
title = {FairAccess: a new Blockchain-based access control framework for the Internet of Things: FairAccess: a new access control framework for IoT},
journal = {Security and Communication Networks},
doi = {10.1002/sec.1748}
}

@inproceedings{blockchainGateway_1_iot,
author = {Cha, Shi-Cho and Tsai, Tsung-Ying and Peng, Wei-Ching and Huang, Tzu-Chia and Hsu, Tzu-Yang},
year = {2017},
month = {10},
pages = {1-3},
title = {Privacy-aware and blockchain connected gateways for users to access legacy IoT devices},
doi = {10.1109/GCCE.2017.8229327}
}

@article{blockchainGateway_2_iot,
author = {Cha, Shi-Cho and Chen, Jyun-Fu and Su, Chunhua and Yeh, Kuo-Hui},
year = {2018},
month = {01},
pages = {1-1},
title = {A Blockchain Connected Gateway for BLE-based Devices in the Internet of Things},
volume = {PP},
journal = {IEEE Access},
doi = {10.1109/ACCESS.2018.2799942}
}

@inproceedings{bbAccessControl,
author = {Maesa, Damiano and Mori, Paolo and Ricci, Laura},
year = {2017},
month = {05},
pages = {206-220},
title = {Blockchain Based Access Control},
isbn = {978-3-319-59664-8},
doi = {10.1007/978-3-319-59665-5_15}
}

@inproceedings{consentManagementIot_2_iot,
author = {Rantos, Konstantinos and Drosatos, George and Ilioudis, Christos and Papanikolaou, Alexandros and Kritsas, Antonios and Demertzis, Konstantinos},
year = {2018},
month = {11},
title = {ADvoCATE: A Consent Management Platform for Personal Data Processing in the IoT Using Blockchain Technology}
}

@inproceedings{consentManagementIot_iot,
author = {Rantos, Konstantinos and Drosatos, George and Demertzis, Konstantinos and Ilioudis, Christos and Papanikolaou, Alexandros},
year = {2018},
month = {07},
pages = {738-743},
title = {Blockchain-based Consents Management for Personal Data Processing in the IoT Ecosystem},
doi = {10.5220/0006911007380743}
}

@inproceedings{iotDataStorage,
 author = {Shafagh, Hossein and Burkhalter, Lukas and Hithnawi, Anwar and Duquennoy, Simon},
 title = {Towards Blockchain-based Auditable Storage and Sharing of IoT Data},
 booktitle = {Proceedings of the 2017 on Cloud Computing Security Workshop},
 series = {CCSW '17},
 year = {2017},
 isbn = {978-1-4503-5204-8},
 location = {Dallas, Texas, USA},
 pages = {45--50}
} 


@article{GDPRCompliantPersonalDM,
  author    = {Nguyen Binh Truong and
               Kai Sun and
               Gyu Myoung Lee and
               Yike Guo},
  title     = {GDPR-Compliant Personal Data Management: {A} Blockchain-based Solution},
  journal   = {CoRR},
  volume    = {abs/1904.03038},
  year      = {2019},
  eprint    = {1904.03038}
}

@inproceedings{ikp_2,
author = {Matsumoto, Stephanos and Reischuk, Raphael},
year = {2015},
month = {01},
pages = {},
title = {Certificates-as-an-Insurance: Incentivizing Accountability in SSL/TLS},
doi = {10.14722/sent.2015.23009}
}

@inproceedings{ikp,
author = {Matsumoto, Stephanos and Reischuk, Raphael},
year = {2017},
month = {05},
pages = {410-426},
title = {IKP: Turning a PKI Around with Decentralized Automated Incentives},
doi = {10.1109/SP.2017.57}
}

@article{_regulation_2016,
  title = {Regulation ({{EU}}) 2016/679 of the {{European Parliament}} and of the {{Council}} of 27 {{April}} 2016 on the Protection of Natural Persons with Regard to the Processing of Personal Data and on the Free Movement of Such Data, and Repealing {{Directive}} 95/46/{{EC}} ({{General Data Protection Regulation}})},
  volume = {L 119/1},
  journal = {Official Journal of the European Union},
  author = {{European Parliament \& Council}},
  month = apr,
  year = {2016},
  keywords = {GDPR},
  pages = {1-88}
}

@techreport{Article29DataProtectionWorkingPartyOpinion2011,
  title = {Opinion 15/2011 on the Definition of Consent},
  number = {01197/11/EN WP187},
  author = {{Article 29 Data Protection Working Party}},
  month = jul,
  year = {2011}
}

@techreport{Article29WorkingPartyGuidelinesconsentRegulation2018,
  title = {Guidelines on Consent under {{Regulation}} 2016/679},
  number = {17/EN WP259 rev.01},
  author = {{Article 29 Data Protection Working Party}},
  year = {2018}
}

@inproceedings{paper_eberhardt_tai_offchaining_patterns,
Title = {{On or Off the Blockchain? Insights on Off-Chaining Computation and Data}},
Author = {J.Eberhardt and S.Tai},
Booktitle = {{ESOCC 2017: 6th European Conference on Service-Oriented and Cloud Computing}},
Year = {2017}
}


@misc{paper_zkSnarks,
    author = {Rosario Gennaro and Craig Gentry and Bryan Parno and Mariana Raykova},
    title = {Quadratic Span Programs and Succinct NIZKs without PCPs},
    howpublished = {Cryptology ePrint Archive, Report 2012/215},
    year = {2012}
}

@misc{flightstats,
title = {Flightstats},
howpublished = {Available at: \url{https://www.flightstats.com/v2/}},
note = { Accessed in February 2019}
}

@misc{etherisc,
title = {Etherisc},
howpublished = {Available at: \url{https://etherisc.com/}},
note = { Accessed in February 2019}
}

@misc{bloGPV,
title = {BloGPV},
howpublished = {Available at: \url{http://www.blogpv.de}},
note = { Accessed in February 2019}
}

@ARTICLE{manInTheMiddle,
author={F. {Callegati} and W. {Cerroni} and M. {Ramilli}},
journal={IEEE Security Privacy},
title={Man-in-the-Middle Attack to the HTTPS Protocol},
year={2009},
volume={7},
number={1},
pages={78-81},
month={Jan}
}

@article{iotLogistics,
author={N. {Kshetri}},
journal={IT Professional},
title={Can Blockchain Strengthen the Internet of Things?},
year={2017},
volume={19}
}

@article{supplyChain_friedhelm,
  author    = {Martin Westerkamp and
               Friedhelm Victor and
               Axel K{\"{u}}pper},
  title     = {Blockchain-based Supply Chain Traceability: Token Recipes model Manufacturing
               Processes},
  journal   = {CoRR},
  year      = {2018}
}

@Article{insuranceBlockchain,
AUTHOR = {Gatteschi, Valentina and Lamberti, Fabrizio and Demartini, Claudio and Pranteda, Chiara and Santamaría, Víctor},
TITLE = {Blockchain and Smart Contracts for Insurance: Is the Technology Mature Enough?},
JOURNAL = {Future Internet},
VOLUME = {10},
YEAR = {2018}
}

@inproceedings{insuranceForCars,
 author = {Vo, Hoang Tam and Mehedy, Lenin and Mohania, Mukesh and Abebe, Ermyas},
 title = {Blockchain-based Data Management and Analytics for Micro-insurance Applications},
 booktitle = {Proceedings of the 2017 ACM on Conference on Information and Knowledge Management},
 series = {CIKM '17},
 year = {2017},
 location = {Singapore, Singapore},
 publisher = {ACM}
}


@inproceedings{TownCrier,
 author = {Zhang, Fan and Cecchetti, Ethan and Croman, Kyle and Juels, Ari and Shi, Elaine},
 title = {Town Crier: An Authenticated Data Feed for Smart Contracts},
 booktitle = {Proceedings of the 2016 ACM SIGSAC Conference on Computer and Communications Security},
 year = {2016},
 publisher = {ACM}
 }

@article{ASTRAEA,
  author    = {John Adler and
               Ryan Berryhill and
               Andreas G. Veneris and
               Zissis Poulos and
               Neil Veira and
               Anastasia Kastania},
  title     = {Astraea: {A} Decentralized Blockchain Oracle},
  journal   = {CoRR},
  year      = {2018}
}

@inproceedings{PoL_nasruli,
  author    = {Bulat Nasrulin and
               Muhammad Muzammal and
               Qiang Qu},
  title     = {A Robust Spatio-Temporal Verification Protocol for Blockchain},
  booktitle = {{WISE} {(1)}},
  series    = {Lecture Notes in Computer Science},
  volume    = {11233},
  pages     = {52--67},
  publisher = {Springer},
  year      = {2018}
}

@inproceedings{PoL_Amoretti,
author={M. {Amoretti} and G. {Brambilla} and F. {Medioli} and F. {Zanichelli}},
booktitle={2018 IEEE International Conference on Software Quality, Reliability and Security Companion (QRS-C)},
title={Blockchain-Based Proof of Location},
year={2018},
month={July}
}

@inproceedings{off-chaining_models_heiss,
 author = {Eberhardt, Jacob and Heiss, Jonathan},
 title = {Off-chaining Models and Approaches to Off-chain Computations},
 booktitle = {Proceedings of the 2Nd Workshop on Scalable and Resilient Infrastructures for Distributed Ledgers},
 series = {SERIAL'18},
 year = {2018},
 publisher = {ACM}
}

@inproceedings{trustworthyOnchaining_heiss,
 author = {Heiss, Jonathan and Eberhardt, Jacob and Tai, Stefan},
 title = {From Oracles to Trustworthy Data On-chaining Systems},
 booktitle = {2019 IEEE International Conference on Blockchain},
 year = {2019},
 organization = {IEEE}
}

@inproceedings{TLS-N,
  author    = {Hubert Ritzdorf and
               Karl W{\"{u}}st and
               Arthur Gervais and
               Guillaume Felley and
               Srdjan Capkun},
  title     = {{TLS-N:} Non-repudiation over {TLS} Enablign Ubiquitous Content Signing},
  booktitle = {{NDSS}},
  publisher = {The Internet Society},
  year      = {2018}
}


@misc{TLSNotary,
author = {TLSNotary},
title = {TLSnotary - a mechanism for independently audited https sessions},
howpublished = {Available at: \url{https://tlsnotary.org/TLSNotary.pdf}},
year = {2014},
note = { Acccessed in February 2019}
}

@misc{Oraclize,
author = {Oraclize},
title = {A Scalable Architecture for On-Demand, Untrusted Delivery of Entropy},
howpublished = {Available at: \url{www.oraclize.it}},
note = { Acccessed in February 2019}
}

@misc{Hivemind,
author = {Paul Sztorc},
title = {Truthcoin: Peer-to-Peer Oracle System and Prediction Marketplace},
howpublished = {Available at: \url{http://www.augur.net/whitepaper.pdf}},
year = {2018},
note = { Acccessed in February 2019}
}

@misc{Augur,
author = {J. Peterson and J. Krug and M. Zoltu and A. K. Williams and S. Alexander},
title = {Augur: a decentralized oracle and prediction market platform},
howpublished = {Available at: \url{http://bitcoinhivemind.com/papers/truthcoin-whitepaper.pdf}},
year = {2015},
note = { Acccessed in February 2019}
}

@misc{Chainlink,
author = {S. Ellis and A. Juels and S. Nazarov},
title = {Chainlink a decentralized oracle network},
howpublished = {Available at: \url{ https://link.smartcontract.com/whitepaper}},
year = {2017},
note = { Acccessed in February 2019}
}

@misc{Gnosis,
author = {S. Ellis and A. Juels and S. Nazarov},
title = {Gnosis whitepaper},
howpublished = {Available at: \url{https://gnosis.pm/resources/default/pdf/gnosis-whitepaper-DEC2017.pdf}},
year = {2017},
note = { Acccessed in February 2019}
}

@misc{iExec,
author = {Gilles Fedak and Wassim Bendella and Eduardo Alves},
title = {iExec: Blockchain-Based Decentralized Cloud Computing },
howpublished = {Available at: \url{https://iex.ec/wp-content/uploads/pdf/iExec-WPv3.0-English.pdf}},
year = {2018},
note = { Acccessed in February 2019}
}

@misc{golem,
author = {Golem},
title = {Golem Project - Crowdfunding Whitepaper},
howpublished = {Available at: \url{https://golem.network/crowdfunding/Golemwhitepaper.pdf}},
year = {2016},
note = { Acccessed in February 2019}
}

@misc{openBazaar,
title = {OpenBazaar},
howpublished = {Available at: \url{https://openbazaar.org}},
note = { Acccessed in February 2019}
}

@misc{Shintaku,
author = {Ryuuji Kamiya},
title = {Shintaku: An End-to-End-Decentralized General-Purpose Blockchain Oracle System},
howpublished = {Available at: \url{https://gitlab.com/shintaku-group/paper/blob/master/shintaku.pdf}},
year = {2018},
note = { Acccessed in February 2019}
}



@article{paper_enigma_Zyskind,
  author    = {Guy Zyskind and
               Oz Nathan and
               Alex Pentland},
  title     = {Enigma: Decentralized Computation Platform with Guaranteed Privacy},
  journal   = {CoRR},
  year      = {2015}
}

@INPROCEEDINGS{decentralizedPrivacy_Zyskind,
author={G. {Zyskind} and O. {Nathan} and A. '. {Pentland}},
booktitle={2015 IEEE Security and Privacy Workshops},
title={Decentralizing Privacy: Using Blockchain to Protect Personal Data},
year={2015},
month={May}
}

@misc{APIdocumentation_intel_AttestationSGX,
	author = {{Intel}},
	title = {{Innovative Technology for CPU Based Attestation and Sealing}},
	howpublished = {\url{https://software.intel.com/en-us/articles/innovative-technology-for-cpu-based-attestation-and-sealing}},
  year = {2013}
}

@article{paper_Brasser_sgxCacheAttack1,
  author    = {Ferdinand Brasser and
               Urs M{\"{u}}ller and
               Alexandra Dmitrienko and
               Kari Kostiainen and
               Srdjan Capkun and
               Ahmad{-}Reza Sadeghi},
  title     = {Software Grand Exposure: {SGX} Cache Attacks Are Practical},
  journal   = {CoRR},
  year      = {2017}
}

@article{paper_schwarz_sgxCacheAttack2,
  author    = {Michael Schwarz and
               Samuel Weiser and
               Daniel Gruss and
               Cl{\'{e}}mentine Maurice and
               Stefan Mangard},
  title     = {Malware Guard Extension: Using {SGX} to Conceal Cache Attacks},
  journal   = {CoRR},
  volume    = {abs/1702.08719},
  year      = {2017}
}

@article{papaer_Moghimi_sgxCacheAttack3,
  author    = {Ahmad Moghimi and
               Gorka Irazoqui and
               Thomas Eisenbarth},
  title     = {CacheZoom: How {SGX} Amplifies The Power of Cache Attacks},
  journal   = {CoRR},
  volume    = {abs/1703.06986},
  year      = {2017}
}

@inproceedings {paper_bulck_foreshadow_sgx_attack,
author = {Jo Van Bulck et al.},
title = {Foreshadow: Extracting the Keys to the Intel {SGX} Kingdom with Transient Out-of-Order Execution},
booktitle = {27th {USENIX} Security Symposium ({USENIX} Security 18)},
year = {2018},
address = {Baltimore, MD},
pages = {991{\textendash}1008},
publisher = {{USENIX} Association}
}

@article{paper_wood_ethereum_yellow,
  title={Ethereum: A secure decentralised generalised transaction ledger},
  author={Wood, Gavin},
  journal={Ethereum Project Yellow Paper},
  year={2014}
}

@article{paper_buterin_ethereum_white,
  title={Ethereum: A next-generation smart contract and decentralized application platform},
  author={Buterin, Vitalik},
  journal={\url{https://github.com/ethereum/wiki/wiki/\%5BEnglish\%5D-White-Paper}},
  year={2014}
}

@article{paper_verifiersDilemma_teutsch,
title = {Demystifying Incentives in the Consensus Computer},
author = {Luu, Loi and Teutsch, Jason and Kulkarni, Raghav and Saxena, Prateek},
journal = {Proceedings of the 22nd ACM SIGSAC Conference on Computer and Communications Security - CCS '15},
pages = {706--719},
year = {2015},
publisher = {ACM}
}

@inproceedings{paper_kosba_hawk,
  title={Hawk: The blockchain model of cryptography and privacy-preserving smart contracts},
  author={Kosba, Ahmed and Miller, Andrew and Shi, Elaine and Wen, Zikai and Papamanthou, Charalampos},
  booktitle={Security and Privacy (SP), 2016 IEEE Symposium on},
  pages={839--858},
  year={2016},
  organization={IEEE}
}

@InProceedings{sybilAttack,
author="Douceur, John R.",
editor="Druschel, Peter
and Kaashoek, Frans
and Rowstron, Antony",
title="The Sybil Attack",
booktitle="Peer-to-Peer Systems",
year="2002",
publisher="Springer Berlin Heidelberg"
}

@inproceedings{paper_eberhardt_zokrates,
Title = {ZoKrates - Scalable Privacy-Preserving Off-Chain Computations},
Author = {Jacob Eberhardt and Stefan Tai},
Booktitle = {IEEE International Conference on Blockchain},
Year = {2018},
Organization = {IEEE}
}

@inproceedings{paper_eberhardt_off-chain_computations,
 author = {Eberhardt, Jacob and Heiss, Jonathan},
 title = {Off-chaining Models and Approaches to Off-chain Computations},
 booktitle = {Proceedings of the 2Nd Workshop on Scalable and Resilient Infrastructures for Distributed Ledgers},
 series = {SERIAL'18},
 year = {2018},
 isbn = {978-1-4503-6110-1},
 location = {Rennes, France},
 pages = {7--12},
 numpages = {6},
 url = {http://doi.acm.org/10.1145/3284764.3284766},
 doi = {10.1145/3284764.3284766},
 acmid = {3284766},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@inproceedings{paper_eberhardt_off-chaining,
  title={On or Off the Blockchain? Insights on Off-Chaining Computation and Data},
  author={Eberhardt, Jacob and Tai, Stefan},
  booktitle={European Conference on Service-Oriented and Cloud Computing},
  pages={3--15},
  year={2017},
  organization={Springer}
}

@inproceedings{decema,
  author    = {Markus Klems and
               Jacob Eberhardt and
               Stefan Tai and
               Steffen H{\"{a}}rtlein and
               Simon Buchholz and
               Ahmed Tidjani},
  title     = {Trustless Intermediation in Blockchain-Based Decentralized Service
               Marketplaces},
  booktitle = {Service-Oriented Computing - 15th International Conference, {ICSOC}},
  year      = {2017}
}

@article{safetyLiveness_Lamport,
 author = {Lamport, L.},
 title = {Proving the Correctness of Multiprocess Programs},
 journal = {IEEE Trans. Softw. Eng.},
 year = {1977}
}

@inproceedings{teutsch_verifiersDilemma,
 author = {Luu, Loi and Teutsch, Jason and Kulkarni, Raghav and Saxena, Prateek},
 title = {Demystifying Incentives in the Consensus Computer},
 booktitle = {Proceedings of the 22Nd ACM SIGSAC Conference on Computer and Communications Security},
 series = {CCS '15},
 year = {2015},
 publisher = {ACM}
}



